Malicious and Low Credibility URLs on Twitter during the AstraZeneca COVID-19 Vaccine Development

We investigate the link sharing behavior of Twitter users following the temporary halt of AstraZeneca COVID-19 vaccine development in September 2020. During this period, we show the presence of malicious and low credibility information sources shared on Twitter messages in multiple languages. The malicious URLs, often in shortened forms, are increasingly hosted in content delivery networks and shared cloud hosting infrastructures not only to improve reach but also to avoid being detected and blocked. There are potential signs of coordination to promote both malicious and low credibility URLs on Twitter. Our findings suggest the need to develop a system that monitors the low-quality URLs shared in times of crisis.

==> sections/analysis_old.tex <==
\section{Results}
% In this section, we present our empirical observations.
We show the basic characteristics of the URLs shared on Twitter (Section~\ref{sec:url_pop}).
Second, we analyze the article content pointed by the URLs, and compare the linguistic patterns of the articles hosted at two most popular news sites (Section~\ref{sec:article_text}).
Third, we report the characteristics of low credibility URLs (Section~\ref{sec:low_credible}) and malicious URLs (Section~\ref{sec:malicious}).
Finally, we show coordination patterns within the groups of users who attempt to promote both low credibility and malicious content (Section~\ref{sec:coordination}).

\subsection{URL Popularity}
\label{sec:url_pop}
Figure~\ref{fig:tweets_url_timeseries} shows a spike in URL mentions on September $9^{th}$.
This is mainly due to the reports of the halt in AstraZeneca vaccine development following a suspected adverse reaction of a trial participant.
There are 23,620 (28\%) messages citing distinct 8,566 URLs on this particular day.
The most popular URLs point mainstream news articles, while the article published in \texttt{statnews.com} received the highest number (1,158) of shares~\footnote{https://www.statnews.com/2020/09/08/astrazeneca-covid-19-vaccine-study-put-on-hold-due-to-suspected-adverse-reaction-in-participant-in-the-u-k/}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/social/tweets_url_timeseries_day.pdf}
    \caption{Number of Twitter URL mentions over time. There is a known gap in the data collection between $27^{th}$-$31^{st}$ Aug.}
    \label{fig:tweets_url_timeseries}
\end{figure}

Our objective is to compare the URL sharing activities across different web domains.
Figure~\ref{fig:top10_domain} shows the number of mentions and users involved in these URL-sharing activities.
The size of the markers in this plot are proportional to the number of URLs associated with the domain.
Figure~\ref{fig:top10_domain_growth} shows the number of URL mentions in the hours after the first mention of a URL on Twitter.
We have multiple observations from these figures.

\begin{figure*}[htbp]
\centering
\begin{tabular}{cc}
     \subfloat[Top-10 shared domains]{
    \includegraphics[width=0.42\linewidth]{images/social/top10_domain_info.pdf}
    \label{fig:top10_domain_info}
    }
   &
     \subfloat[Twitter lifespan of URLs by domain]{
     \includegraphics[width=0.58\linewidth]{images/social/top10_domain_growth_median.pdf}
     \label{fig:top10_domain_growth}
     }
     \\
\end{tabular}
	 \caption{Twitter sharing characteristics of most popular domains. Figure a) shows the Top-10 domains by the number of distinct URLs. The size of the markers in this plot are proportional to the number of URLs  associated  with  the  domain. Figure b) shows the number of URL mentions posted at each hour after the first appearance of URL in the respective domain. We count the number of mentions for each URL in the respective hour, and calculate the median number of mentions for the domain of the URL.}
	 \label{fig:top10_domain}
\end{figure*}

First, \texttt{sputniknews.com} is the most popular web domain by the number of mentions (22,251), the number of users (4,358) and the number of URLs (6,638).
However, \texttt{sputniknews.com} URL is not the most popular to be shared in the immediate hours after its first appearance as shown in Figure~\ref{fig:top10_domain_growth}.
For example, the median number of \texttt{sputniknews.com} URL mentions is 2 in an hour.
\texttt{sputniknews.com} is frequently described as a Russian propaganda outlet that spreads master narratives in the Russia's disinformation campaign against the AstraZeneca vaccine development~\cite{newsguard_2021}.



Second, one would expect that the volume of mentions of a web domain and the number of users who share URLs from that domain are correlated with the number of distinct URLs from that domain. 
% thus the domains that appear in Table~\ref{tbl:top10_domains_URLs} appear in Figure~\ref{fig:topk_domain_info}. 
However, \texttt{rt.com}, and \texttt{statnews.com} are media sites that have unexpected popularity for the relatively small content shared (the number of \textsc{url}s). 
While \texttt{statnews.com} is a well recognized American health-oriented news website, \texttt{rt.com} is directly handled by the Russian state media who promotes its own vaccine ("Sputnik V") development~\cite{rory2020vaccinefirstdraft}.
We noticed that \texttt{rt.com} acquires its many mentions from very few URLs: 119 URLs are cited in 3,225 messages during our observation period.
\texttt{rt.com} URLs have the highest number of mentions in the first hour after publication (as shown in Figure~\ref{fig:top10_domain_growth}) relatuve to the rest of popular web sites.
We also noticed \texttt{statnews.com} URLs gain a sudden popularity between 17th to 28th hours after the first URL mention.

Third, we also discovered URLs from two Russian news media domains, \texttt{sputnik-abkhazia.ru} and \texttt{moskva-tyt.ru} that are shared by very few users.
For example, \texttt{sputnik-abkhazia.ru} is the fourth most popular web domain by the number of URLs cited on Twitter messages.
% However, there are only 4 users who cited these URLs (175) in 305 messages, repeatedly.
These URLs are shared solely by the Twitter account controlled by the news media site.
However, they gain limited engagement with other users.
% These messages are in Russian

% Fourth, URLs from the most popular domains are shared on Twitter for more than 24 hours as shown in Figure~\ref{fig:top10_domain_growth}.


% While there is a \texttt{statnews.com} URL active on Twitter for a maximum of 43 hours, there is a \texttt{sputniknews.com} URL cited repeatedly on Twitter messages for more than 8 days.





\subsection{Article Text}
\label{sec:article_text}
% There are 26,422 distinct URLs across 6,990 domains shared on Twitter messages.
% For additional analysis, we scrape the web page content pointed by the URLs using a Python library, Newspaper.
For additional analysis, we scrape the web page content pointed to an URL using a Python library, Newspaper.
We managed to scrape 22,856 articles, where the tool failed to extract content from some web domains mainly due to inactive web pages, and the regulations enforced by the web domain.

According to the Langid~\cite{lui2012langid}, the majority of the articles are in English (6,453) and Spanish (5,197) languages.
Other articles are written in Turkish (1,839), French (1,539), Portuguese (1,277), Russian (784), Italian (772), Greek (708), Japanese (702), Croatian (447), etc.
As shown in Table~\ref{tab:lang_domain}, \texttt{sputniknews.com} has a network of media outlets that publish articles in many languages.
For example, 1,377 and 1,080 \texttt{sputniknews.com} articles are published in Turkish and French.
On the other hand, videos hosted at \texttt{youtube.com} are also found to be in different languages.
For example, 274 and 165 videos shared on Twitter have the title written in English and Spanish languages, respectively.

To analyze the linguistic patterns of the words used in the articles, we use LIWC to count the words associated with different psychological categories.
LIWC~\cite{tausczik2010psychological} is a linguistic dictionary that contains 4,500 words categorized to analyze psycholinguistic patterns in text. 
We use six categories in the LIWC dictionary: Social processes, Affective processes, Cognitive processes, Perceptual processes, Biological processes and Relativity.
% to analyze psycholinguistic patterns in text.
% Empath~\cite{fast2016empath} is a tool that uses deep learning and word embeddings to build a semantically meaningful lexicon for concepts.
% We select 12 categories (surprise, confusion, trust, hate, deception, anger, sympathy, joy, sadness, fear, disappointment, disgust) to cover the emotional words used in the article text.


% We collect 22,856 articles (87\%) for our analysis.
% The tool failed to extract content from 3,566 URLs due to multiple reasons.
% First, the majority of missing articles are from social media web sites (e.g., \texttt{instagram.com, facebook.com etc.}) that do not allow to extract web page content using third party tools.
% Second, some web pages pointed by the URLs are not available.


% en    6453
% es    5197
% tr    1839
% fr    1539
% pt    1277
% ru     784
% it     772
% el     708
% ja     702
% hr     447

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1\linewidth]{images/social/lang_domain_5_edited.pdf}
%     \caption{Five most popular article domains for each language. The size of the circle is proportionate to the number of articles published by the respective domain.}
%     \label{fig:lang_domain}
% \end{figure}

\begin{table*}[htbp]
    \centering
    \caption{The most popular domains hosting articles written in multiple languages. \texttt{sputniknews.com} and \texttt{youtube.com} are among the most popular domains.}
    \label{tab:lang_domain}
    \begin{tabular}{|c|}
    \hline
English  \\ \hline \hline
\textbf{sputniknews.com} \\ \hline
\textbf{youtube.com} \\ \hline
reuters.com \\ \hline
newsfilter.io \\ \hline
nytimes.com \\ \hline
    \end{tabular}
    \begin{tabular}{|c|}
    \hline
Spanish  \\ \hline \hline
\textbf{sputniknews.com} \\ \hline
\textbf{youtube.com} \\ \hline
rt.com \\ \hline
reuters.com \\ \hline
wp.me \\ \hline
    \end{tabular}
    \begin{tabular}{|c|}
    \hline
Turkish  \\ \hline \hline
\textbf{sputniknews.com} \\ \hline
\textbf{youtube.com} \\ \hline
ntv.com.tr \\ \hline
is.gd \\ \hline
sozcu.com.tr \\ \hline
    \end{tabular}
        \begin{tabular}{|c|}
    \hline
French  \\ \hline \hline
\textbf{sputniknews.com} \\ \hline
cvitrolles.wordpress.com \\ \hline
\textbf{youtube.com} \\ \hline
francetvinfo.fr \\ \hline
lalibre.be \\ \hline
    \end{tabular}
    \begin{tabular}{|c|}
    \hline
Portugese  \\ \hline \hline
\textbf{sputniknews.com} \\ \hline
brasil247.com \\ \hline
evsarteblog.wordpress.com \\ \hline
\textbf{youtube.com} \\ \hline
tvi24.iol.pt \\ \hline
    \end{tabular}
\end{table*}

Our objective is to compare and contrast the linguistic patterns used in the misleading and credible news articles.
We used the articles hosted at two most popular domains \texttt{sputniknews.com} and \texttt{reuters.com} for this analysis.
While we know \texttt{sputniknews.com} publishes misleading, questionable content, \texttt{reuters.com} is a credible mainstream news media outlet.
Figure~\ref{fig:liwc_news_articles} shows the fraction of words used in the articles for each LIWC category.
For this comparison, we only used the articles written in English.

% According to Empath, there are more words related to "Trust" lexical category in both news sources (Figure~\ref{fig:empath_news_articles}).
% We believe this is due to the journalism practice of promoting the newsworthiness via building trust~\cite{trilling2017newsworthiness}.

% satire, hoaxes, clickbait and propaganda


It is interesting to note the lack of words used in \texttt{sputniknews.com} articles to cover the main discussion topics related to the biological processes compared to what reported in \texttt{reuters.com} (Figure~\ref{fig:liwc_news_articles}).
We noticed \texttt{sputniknews.com} articles used more words that are associated with social processes (e.g., friends, family), affective processes (e.g., anxiety, sadness), and cognitive processes (e.g., discrepancy, tentative) than what are used in the articles published by \texttt{reuters.com}.
This suggests that the \texttt{sputniknews.com} articles used a deceptive language in their articles while \texttt{reuters.com} articles has a more factual style.
% \shnote{Write more..} \nabeel{We need to provide some interpretation of Figure 3. What can we tell from this linguistic pattern analysis?}

% \begin{figure}[htbp]
% \centering
% \begin{tabular}{c}
% %      \subfloat[Emotional Categories]{
% %     \includegraphics[width=0.48\linewidth]{images/social/empath_news_articles.pdf}
% %     \label{fig:empath_news_articles}
% %     }
% %   &
%      \subfloat[Psycholinguistic Categories]{
%      \includegraphics[width=0.98\linewidth]{images/social/liwc_news_articles.pdf}
%      \label{fig:liwc_news_articles}
%      }
%      \\
% \end{tabular}
% 	 \caption{Lexical patterns used in the articles hosted at \texttt{sputniknews.com} and \texttt{reuters.com}}
% 	 \label{fig:article_content_features}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{images/social/liwc_news_articles.pdf}
    \caption{Lexical patterns used in the articles hosted at \texttt{sputniknews.com} and \texttt{reuters.com}}
    \label{fig:liwc_news_articles}
\end{figure}


\subsection{Low-credibility Information Sources}
\label{sec:low_credible}
In this section, we report how Twitter users react to low-credibility information sources.
We group the web domains according to the classification made by Media Bias/ Fact Check (MBFC)~\cite{mbfc}.
We also cross-check these domains with the list of web sites that publish False COVID-19 information as identified by NewsGuard~\cite{newsguard_2021}.
We identify 6,860 (26\%) URLs from 17 low-credibility information sources that are shared on 26,220 (31\%) messages (as shown in Table~\ref{tab:basic_char_mbfc}).
We note a larger number of URLs published by \texttt{sputniknews.com} compared to other information sources.
% On average, a user share at least five messages citing a \texttt{sputniknews.com} URL.
We believe this may be an example of propaganda technique where the propagandists employ deception, not necessarily via fabrication, but sometimes with concrete evidence, to win public support for their cause~\cite{bernays1928manipulating}.
We also note that Twitter messages share the same article heading in the messages when they cite the same URL.
These users might promote certain topics through massive repetition of messages via injecting URLs.
For example, an article published in \texttt{zerohedge.com} was in the Top-10 most popular URLs on the day when AstraZeneza vaccine development halted~\footnote{https://www.zerohedge.com/markets/ft-confirms-astrazeneca-covid-19-vaccine-caused-serious-spinal-issues-test-patient}.
However, this article tried to build an alternative frame highlighting a statement by the US House Speaker Nancy Pelosi about the issue instead of reporting the details of the main event.
This technique can spoof the Twitter trending algorithm to broadcast their message towards a wider audience and to establish their preferred narrative via artificial amplification.





\begin{table}[htbp]
    \centering
        \caption{Twitter sharing characteristics for low-credible URLs as identified by MBFC and NewsGuard (NG). We use the~\checkmark~mark to reflect whether the domain is being listed as a low-credibility information source by the respective fact checking organization.}
    \label{tab:basic_char_mbfc}
    \scalebox{0.8}{
    \begin{tabular}{|c|c|c|r|r|r|}
    \hline
         Domain &  MBFC & NG & \# Mentions & \# Users & \# URLs \\\hline \hline
 sputniknews.com & \checkmark & \checkmark  & 22,251 & 4,358 & 6,638 \\ \hline
rt.com & \checkmark & \checkmark  & 3,225 & 1,922 & 119 \\ \hline
zenith.news & \checkmark & - & 117 & 6 & 62 \\ \hline
zerohedge.com & \checkmark & \checkmark  & 278 & 249 & 15 \\ \hline
swarajyamag.com & \checkmark & - & 228 & 105 & 5 \\ \hline
oann.com & \checkmark & \checkmark  & 50 & 48 & 4 \\ \hline
childrenshealthdefense.org & \checkmark & \checkmark  & 3 & 3 & 3 \\ \hline
globalresearch.ca & \checkmark & \checkmark  & 16 & 7 & 3 \\ \hline
torontotoday.net & \checkmark & - & 9 & 5 & 2 \\ \hline
gnews.org & \checkmark & \checkmark  & 4 & 4 & 2 \\ \hline
truepundit.com & \checkmark & \checkmark  & 29 & 29 & 1 \\ \hline
needtoknow.news & \checkmark & - & 5 & 5 & 1 \\ \hline
oye.news & \checkmark & \checkmark  & 1 & 1 & 1 \\ \hline
gellerreport.com & \checkmark & \checkmark  & 1 & 1 & 1 \\ \hline
barenakedislam.com & \checkmark & - & 1 & 1 & 1 \\ \hline
wakingtimes.com & \checkmark & \checkmark  & 1 & 1 & 1 \\ \hline
thegatewaypundit.com & \checkmark & \checkmark  & 1 & 1 & 1 \\ \hline
    \end{tabular}
    }
\end{table}


\subsection{Malicious URLs}
\label{sec:malicious}
% \shnote{we can add infra level analysis here.}
We use VirusTotal (VT) \cite{VirusTotal} to extract the \textit{maliciousness} of URLs.
VT provides the state-of-the-art aggregated intelligence for domains and URLs, and relies on more than 70 third-party updated antivirus (AV) engines.
 For all distinct URLs in our collection, we extract VT scan  reports via querying the publicly available API.
Each VT scan report contains of the verdict from every AV engine, information related to the URL such as first and last seen dates of the URL in the VT system, hosting IP address,  final redirected URL (if applicable), content length, etc.  
% We submitted all URLs to the Virustotal scan via APIs and collected the scan reports for both windows and checked the positive count of each scan. 
%We use the number of Antivirus engines that mark a URL \textit{maliciousness} as a feature to distinguish good and bad URLs. 
Each AV engine in a VT report detects if the URL is malicious or not. We use the number of engines that detect a URL as malicious as an indication of maliciousness of the URL.

%\shnote{Edit from here.}
In this study, we label a URL as malicious if at least one AV engine, that is \#VT $\ge$ 1, detects it as malicious. We identify 441 
% \nabeel{(Updated from 343 to 441 as the numbers show this)}
malicious URLs from the collected VT reports. We observe that 25.75\% of the malicious URLs utilize URL shortening services with top 4 services being bit.ly, tinyurl.com, ow.ly and goo.su whereas as only 0.97\% of benign URLs utilize such services.  This observation is consistent with the trend that miscreants increasingly utilize shortening services to camouflage malicious URLs presenting non-suspecting URLs to users~\cite{fas2020malware}. 
% This in turn increases the likelihood of users clicking on such links and becoming victims. The Alexa rank~\cite{alexa} of a domain indicates its access popularity. 
We find that 30.80\% of the domains related to malicious URLs are ranked below 100K by Alexa~\cite{alexa} (The lower the rank value, the higher the popularity). This indicates the concerning fact miscreants are able to reach a large user base reaping a high return on investment for their attacks.

We further analyze the malicious URLs to identify related malicious URLs. To this end, based on the lexical features in the literature and the hosting features mentioned in Table~\ref{tab:infra_features}, we cluster the malicious URLs using PCA/OPTICS algorithm~\cite{scikit-learn}. While lexical features identify characteristics related to URLs themselves, hosting features, extracted from Farsight Passive DNS (PDNS) data~\cite{dnsdb}, capture the characteristics of underlying hosting infrastructure. As shown in Figure~\ref{fig:t-sne-all}, these features collectively identify 10 distinct malicious URL clusters. We manually verified the accuracy of the top 2 clusters by checking the web page content, registration information and domain certificate information. 
Our observations suggest that attackers launch multiple attacks at the same time.
We also analyze the clusters based on the maliciousness of URLs.
%Figure~\ref{fig:t-sne-all} shows the 3 dimensional t-SNE visualization of the clustered domains. 
The maliciousness of a URL can loosely be measured by \#VT, the number of VT positives. An interesting observation is that URLs belonging to different maliciousness levels share similar lexical and hosting features.   


We further analyze these malicious URLs in terms of where they are hosted. To our surprise, we find that 80.04\% of these malicious URLs are hosted in CDNs such as Cloudflare and Akamai. While CDNs provide fast delivery of content across the globe through their distributed computing infrastructure, we believe a key reason why miscreants utilize such services is to improve attack agility and stay below the radar of malicious domain detection mechanisms in place. This observation is further reinforced with the increased utilization of public cloud computing infrastructure (33.5\% of all malicious URLs) sharing hosting IPs with tens of thousands of unrelated domains, which are mostly benign. Such shared IPs are usually not blocked in practice due to the collateral damage.

%We extracted the URLs that VirusTotal positive count is greater than 0 and ran the t-SNE clustering \ref{fig:t-sne-all} on extracted features described in the table \ref{tab:infra_features}. 
%The cluster projection of the 3 dimension space shows a clear difference in differncet VT positive levels which indicated the correlations of each group. And another observation that we could expose ourselves was these malicious domains (\#VT>0) had a high likelihood of using content delivery networks. It’s ambiguous to clearly mention the usage of content delivery networks. 
%It could be fast delivery of their website across the world or misuse the anonymity provided by the content delivery networks.
% \shnote{Can we explain these numbers in more details, connecting with the implications? given the numbers at Table~\ref{tab:server_char}, what can we derive? For example, what special about hiding behind cloudfare?} \nabeel{I am not sure what insights we can infer from the web server distribution other then the fact that attackers are utilizing open source web servers mainly.}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/infra/t-sne-aug.png}
%     \caption{T-sne of Aug}
%     \label{fig:t-sne-aug}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/infra/t-sne-sep.png}
%     \caption{T-sne of sep}
%     \label{fig:t-sne-sep}
% \end{figure}
 \begin{table}[htbp]
\caption{Details of the hosting features for the malicious URL clustering} %\nabeel{This is predominantly lexical features, not infrastructure features. We need to update this unless we add pdns (hosting) features}}
\label{tab:infra_features}
\begin{tabular}{|l|l|}
\hline
\textbf{Feature}   & \textbf{Description}                                                                             \\ \hline \hline
%\multicolumn{2}{|c|}{\textbf{Lexical Features}}\\
%\hline
%\#Subdomains   & Number of levels in subdomain part of the FQDN                                          %\\ \hline
%Minus          & Number of dashes appear in the FQDN %                                                    \\ \hline
%BrandIs        & Is it impersonating a popular Alexa top 1000 brand?                                     \\ \hline
%Similar        & Is the domain contains words within Levenshtein distance 2 of a popular Alexa top brand \\ \hline
%Fake\_TLD      & Does the domain name includes a fake gTLD (com, edu, net, org, gov)?                    \\ \hline
%Pop\_Keywords  & Does the domain name includes popular keywords?                                         \\ \hline
% \#VT positives & Number of AV engine marked as malicious                                                 \\ \hline
%\multicolumn{2}{|c|}{\textbf{Hosting Features}}\\
%\hline
VT\_Dur    & URL duration in VT                                    \\ \hline
PDNS\_Dur & Domain duration in PDNS \cite{Exposure_Bilge2014}\\ \hline
\#IPs & Number of hosting IPs during the study period \\ \hline
\#Queries & Number of times the domain is accessed \\ \hline
\#NSes & Number of Name servers \\ \hline
Is\_NS & NS domain matches the domain name? \\ \hline
\#SOAs & Number of administrative domains \\ \hline
Is\_SOA & Admin domain matches the domain name? \\ \hline
\#Domains & Number of domains hosted on the IP \\ \hline
\#Queries\_IP & Number of times the IP is accessed \\ \hline
ASN & Autonomous System Number \\ \hline
Org & Organization owning the ASN \\ \hline
%Total          & Total AV engines involved                                                               \\ \hline
\end{tabular}
\end{table}


%\begin{figure}[h]
%\begin{subfigure}{0.45\linewidth}
%\includegraphics[width=\linewidth]{images/infra/clusters_optics.png} 
%\caption{Clusters in General}
%\label{fig:optics}
%\end{subfigure}
%\begin{subfigure}{0.45\linewidth}
%\includegraphics[width=\linewidth]{images/infra/t-sne-all.png}
%\caption{Clusters Colored based on maliciousness level}
%\label{fig:t-sne-all}
%\end{subfigure}
%\caption{Malicious URL Clusters}
%\label{fig:clusters}
%\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{images/infra/clusters_optics.png}
    \caption{Malicious URL clusters based on the lexical and hosting features. Each point is a URL, and colored according to the cluster it belongs.}
    \label{fig:t-sne-all}
\end{figure}

% \begin{table}[htbp]
% \caption{Server Characteristics for malicious URLs}
% \label{tab:server_char}
% \begin{tabular}{|l|l|l|}
% \hline
% Server            & \# URLs & \% URLs \\ \hline \hline
% nginx      & 96     & 21.573\%                 \\ \hline
% undetected         & 87     & 19.550\%                 \\ \hline
% cloudflare             & 83    & 18.651\%                \\ \hline
% Apache & 55     & 12.359\%                 \\ \hline
% openresty     & 18     & 4.044\%                 \\ \hline
% LiteSpeed        & 13    & 2.921\%                \\ \hline
% \end{tabular}
% \end{table}


% VT ==1 server detection September

% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% Server               & Count & percentage from dataset \\  \hline \hline
% LiteSpeed            & 10    & 3.649\%                 \\ \hline
% openresty            & 9     & 3.284\%                 \\ \hline
% undefined            & 66    & 24.087\%                \\ \hline
% Sucuri/Cloudproxy    & 6     & 2.189\%                 \\ \hline
% Apache/2.2.31 (Unix) & 6     & 2.189\%                 \\ \hline
% nginx                & 54    & 19.708\%                \\ \hline
% cloudflare           & 50    & 18.248\%                \\ \hline
% \end{tabular}
% \end{table}







\subsection{User Co-sharing Practices}
\label{sec:coordination}
% \shnote{drafts.}
As reported previously~\cite{starbird2019collaborative,pacheco2020uncovering}, there are signs of coordination to spread the disinformation content.
% Pacheco et al.~\cite{pacheco2020uncovering} discovered that a group of Twitter accounts retweet the same tweet to promote certain narratives in this context.
% We extend the coordination framework developed by Pacheco et al.~\cite{pacheco2020uncovering}. 
% utilizing the URL sharing activities by Twitter users.
In this work, one of our assumptions is that the coordination is based on the content being shared (i.e., URLs mentioned in the tweets).
One of our objectives is to measure the extent of coordination in URL sharing activities.
% that leads to any form of echo chamber effects at the end.
We construct two bipartite networks to quantify the amount of such coordination effort.
The first network connects an author to a low credible URL mentioned in a tweet, and the second network connects an author to a malicious URL mentioned in a tweet.
These networks would capture any suspicious behavior of promoting a particular URL. 
% while the user-domain network would capture any sustained effort to amplify a particular information source.
% We also construct two random bi-partite networks using the Newman's configuration model~\cite{newman2003structure} for the comparison.
% Given the original user-URL bi-partite network, we match the two degree sequences in the users and URLs in the random bi-partite network.
% choose pairs of stubs at random from
% the network and connect them together

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.4\linewidth]{images/social/nx_bi_user_url_vul.png}
%     \caption{Bi-partite network between Users (white) and malicious URLs (red) as identified by VirusTotal.}
%     \label{fig:bi_user_vul_urls}
% \end{figure}


\paragraph{User-(low-credible) URLs Bipartite Network}
We identify 6,860 low-credible information URLs that are shared by 6,600 users in 26,220 Twitter messages.
The five (0.08\%) most active users cite low-credible URLs in 6,404 (24\%) messages.
Their most preferred information source is \texttt{tr.sputniknews.com} which is the Turkish outlet of the sputnik media network.
  

\paragraph{User-(malicious) URLs Bipartite Network}

\begin{figure*}[htbp]
\centering
\begin{tabular}{cc}
     \subfloat[Coordination to promote low-credible URLs (KS=0.6,p-value=0.001)]{
    \includegraphics[width=0.48\linewidth]{images/social/bipartite_clustering_user_mbfc_url.pdf}
    \label{fig:bipartite_clustering_user_mbfc_url}
    }
   &
     \subfloat[Coordination to promote malicious URLs (KS=0.27,p-value=4.45$e^{-12}$)]{
     \includegraphics[width=0.48\linewidth]{images/social/bipartite_clustering_user_mal_url.pdf}
     \label{fig:bipartite_clustering_user_mal_url}
     }
     \\
\end{tabular}
	 \caption{Bipartite clustering coefficient of a) the user-(low credible) URL network, b) the user-(malicious) URL network. We also compare the network clustering values with a random bipartite network using the Newman's configuration model~\cite{newman2003structure}. The deviation of the clustering values from the random bipartite network shows potential coordination effort to promote these URLs on Twitter.}
	 \label{fig:bipartite_clustering}
\end{figure*}

We identify 441
%\nabeel{Should this also be 441?}
malicious URLs that are shared by 357 users in 571 Twitter messages.
% Figure~\ref{fig:bi_user_vul_urls} shows the bi-partite network between users (white) and malicious URLs (red).
While a user might share a malicious URL unwittingly, it is suspicious to note users who share multiple malicious URLs.
Specifically, we identify 51 users who share more than 1 malicious URL, and 21 users who share more than 2 malicious URLs.
% As previously noted~\cite{fas2020malware} and observe above, many such URLs are packaged inside shortened URLs (e.g., bit.ly, tinyurl.com, shar.es, cutt.ly, ow.ly)


Figures~\ref{fig:bipartite_clustering_user_mbfc_url} and ~\ref{fig:bipartite_clustering_user_mal_url} show the distributions of bipartite clustering coefficients~\cite{latapy2008basic} for URLs in the two bipartite networks respectively.
% This clustering coefficient is proposed for two-mode networks by Latapy et al.~\cite{latapy2008basic}.
Clustering coefficient values are higher for URLs when they are shared by a group of users who engage with other URLs together.
We compare the similar clustering values which are calculated from the identical random bipartite networks.
We construct two random bipartite networks using the Newman's configuration model~\cite{newman2003structure} for the comparison.
Given the original user-URL bipartite network, we match the two degree sequences in the users and URLs in the random bipartite network.
% These networks are constructed according to Newman's configuration model (as described in Section~\ref{sec:coordination}).
We noticed a significant deviation of clustering coefficient values for URLs in both bipartite networks compared to URLs in the random bipartite networks (as shown Figures~\ref{fig:bipartite_clustering_user_mbfc_url} and~\ref{fig:bipartite_clustering_user_mal_url}).
For example, there are 4,320 (63\%) low-credibility URLs with a clustering coefficient value greater than 0.8 than those number of URLs (217) in the random bipartite network.
In the malicious URL network, there are 121 URLs with a clustering coefficient value greater than 0.8 that are promoted by the same set of users (the expected number of URLs is 36 in the random network).

To confirm our observation, we also perform the Kolmogorov-Smirnov (KS) test between the clustering coefficient values from the original and random bipartite networks.
KS-statistic values (statistically significant) are 0.6 and 0.27 for the low-credibility URL network and malicious URL network, respectively.
This suggests the sustained effort of users to amplify both misleading and malicious content.
There may be different types of users (e.g., bots, cyborgs, paid activists) who amplify these URLs.
That would remain as a future work to identify these types of users.









==> sections/keyfindings.tex <==
% \section{Key Findings}
% This study provides an in-depth analysis of a Twitter dataset around AstraZeneca COVID vaccine development released as a part of Grand Challenge\footnote{https://www.insna.org/nasn-2021-grand-challenge}, North American Social Network Conference, 2021. 
% In brief, we show:
% \begin{enumerate}
%  \item the presence of malicious and low credibility information sources shared on Twitter messages in multiple languages.
%      \item %\shnote{Nabeel, please add the key findings from the URL clustering using infra features}
%       the malicious URLs, often in shortened forms, are increasingly hosted in content delivery networks and shared cloud hosting infrastructures not only to improve reach but also to avoid being detected and blocked.
%     \item potential signs of coordination to promote both malicious and low credibility URLs on Twitter. We use a null model and several statistical tests to identify meaningful coordination behavior.
% \end{enumerate}


==> sections/related.tex <==
\section{Related Work}
\shnote{Need to fix.}
% URL lifespan is determined to a large extent by the type of con- tent, the source of its origin also impacts its persistence~\cite{wu2011says}.
% ~\cite{baly2020written} show the content of the news articles is useful for predicting the factuality and the political bias of news articles.
~\cite{samory2020characterizing} characterize 639 news sources, both credible and questionable, according to the audience that shares their articles on Twitter.
They identified four communities, one is home to mainstream, high-circulation sources from all sides of the political spectrum; one to satirical, left-leaning sources; one to bipartisan conspiratorial, pseudo-scientific sources; and one to right-leaning, deliberate misinformation sources.
Further, they show how the news articles shared on Twitter differ across the four groups along linguistic and psycholinguistics measures.

False information (propaganda, hoax, clickbait, and satire) has different emotional patterns in each of its types, and emotions play a key role in deceiving the reader~\cite{ghanem2020emotional}.
The results show that the detection of suspicious news in Twitter is harder than detecting it in news articles.

% ~\cite{vosoughi2018spread} investigated a corpus of true and false tweet rumors from different aspects. From an emotional point of view, they found that false rumors inspired fear, disgust, and surprise in their replies while the true ones inspired joy and anticipation.

% found that real tweets contain significantly fewer bias markers, hedges, subjective terms, and less harmful words. They also found that propaganda news targets morals more than satires and hoaxes but less than clickbaits.
There several studies ~\cite{Exposure_Bilge2014} ~\cite{ravindu2021compromised} to identity the malicious urls using infrastructure features. ~\cite{austin2020infrastructure} used infrastructure features to identify the Disinformation Websites.   
